Second-order accurate normal reconstruction from volume fractions on unstructured meshes with arbitrary polyhedral cells

This paper introduces a novel method for the efficient second-order accurate computation of normal fields from volume fractions on unstructured polyhedral meshes. Locally, i.e. in each mesh cell, an averaged normal is reconstructed by fitting a plane in a least squares sense to the volume fraction data of neighboring cells while implicitly accounting for volume conservation in the cell at hand. The resulting minimization problem is solved approximately by employing a Newton-type method. Moreover, applying the Reynolds transport theorem allows to assess the regularity of the derivatives. Since the divergence theorem implies that the volume fraction can be cast as a sum of face-based quantities, our method considerably simplifies the numerical procedure for applications in three spatial dimensions while demonstrating an inherent ability to robustly deal with unstructured meshes. We discuss the theoretical foundations, regularity and appropriate error measures, along with the details of the numerical algorithm. Finally, numerical results for convex and non-convex hypersurfaces embedded in cuboidal and tetrahedral meshes are presented, where we obtain second-order convergence for the normal alignment and symmetric volume difference. Moreover, the findings are substantiated by completely new deep insights into the minimization procedure.

==> 03_99_spline_approximation.tex <==
%
% Spline-based approximation
%
\subsubsection{A spline-based approximation approach}
\begin{remark}[Connectivity]
In cases where establishing edge- or vertex neighborhoods is infeasible, this approach may come in handy. %
\end{remark}
As has been shown in \citet{JCP_2021_fbip}, the volume fraction in any polyhedron can be approximated by a cubic spline via
\begin{align}
\polyvof_k\fof{\signdistref}\approx%
\begin{cases}%
0&\text{if}\quad\signdistref<\projvertpos{-,k},\\%
3\tilde{\signdist}_k^2-2\tilde{\signdist}_k^3&\text{if}\quad\signdistref\in[\projvertpos{-,k},\projvertpos{+,k}],\\%
1&\text{if}\quad\signdistref>\projvertpos{+,k},\\%
\end{cases}
\quad\text{with}\quad%
\tilde{\signdist}_k\defeq\frac{\signdistref-\projvertpos{-,k}}{\projvertpos{+,k}-\projvertpos{-,k}}.%
\end{align}
\begin{figure}[htbp]
\null\hfill%
\includegraphics{algorithm_initial_value}%
\hfill\null%
\caption{Cubic spline approximation of volume fraction for cube.}
\end{figure}

The signed distance $\signdistref$ must be chosen to match the prescribed volume fraction $\polyvofdata_0$ in the stencil center, i.e. %
\begin{align}
\polyvof_0\fof{\signdistref}\stackrel{!}{=}\polyvofdata_0%
\quad\implies\quad%
\signdistref=\projvertpos{-,0}+\brackets{\projvertpos{+,0}-\projvertpos{-,0}}\brackets*{\frac{1}{2}-\cos\brackets*{\frac{\arccos\fof{2\polyvofdata_0-1}-2\pi}{3}}},%
\end{align}
where $\signdistref$ as well as the bounds $\projvertpos{\pm,k}$ are continuous functions of the normal $\plicnormal$. \refFig{spline_approx_illustration} illustrates the concept in two spatial dimensions. %
\begin{figure}[htbp]
\null\hfill%
\includegraphics[page=1]{spline_illustration}%
% \hfill%
% \includegraphics[page=2]{spline_illustration}%
% \hfill\null%
\hfill% \\%
% \null\hfill%
\includegraphics[page=3]{spline_illustration}%
\hfill%
\includegraphics[page=4]{spline_illustration}%
\hfill\null%
\caption{Spline approximation in a triangular stencil.}%
\label{fig:spline_approx_illustration}%
\end{figure}


==> 05_99_qualitative_analysis.tex <==
\subsection{Qualitative assessment}
\begin{figure}[htbp]%
\null\hfill%
\includegraphics[page=1]{cuboidmesh_0020_comparison}%
\hfill%
\includegraphics[page=3]{cuboidmesh_0020_comparison}%
\hfill\null%
\\%
\null\hfill%
\includegraphics[page=3]{cuboidmesh_0020_comparison}%
\hfill%
\includegraphics[page=4]{cuboidmesh_0020_comparison}%
\hfill\null%
\caption{Comparison of reconstruction algorithms for prolate ellipsoid on cuboid mesh ($N=20$; cf.~\reftab{mesh_characteristics}).}%
\end{figure}

\begin{figure}[htbp]%
\null\hfill%
\includegraphics[page=1]{tetmesh_0020_comparison}%
\hfill%
\includegraphics[page=3]{tetmesh_0020_comparison}%
\hfill\null%
\\%
\null\hfill%
\includegraphics[page=3]{tetmesh_0020_comparison}%
\hfill%
\includegraphics[page=4]{tetmesh_0020_comparison}%
\hfill\null%
\caption{Comparison of reconstruction algorithms for prolate ellipsoid on tetrahedron mesh ($N=20$; cf.~\reftab{mesh_characteristics}).}%
\end{figure}
